The most entangled states of four and seven qubits

Pure states of four and seven qubits cannot be maximally entangled across every balanced bipartition; we determine how entangled they can be on average. For four qubits we prove the conjecture of Higuchi and Sudbery: the mean von Neumann entropy of the three $2|2$ cuts is at most $1+\tfrac12\log_2 3$ bits, with equality exactly on the local-unitary orbits of their state $M_4$ and its complex conjugate. For seven qubits the mean purity of the 35 balanced $3|4$ cuts is at least $121/917$ and their mean entropy is at most $2.965356029\ldots$ bits, each with a unique optimiser up to local unitaries and qubit permutations. The two optimisers are distinct members of one icosahedral family, so minimum purity and maximum entropy select different states. The proofs bound moments of the marginal spectra by positive identities on several copies of the state, some of them spin flipped, and bound the entropy by a polynomial in those moments. The four-qubit maximum has an analytic proof; the seven-qubit proofs, and some of the four-qubit refinements below, are computer-assisted, with exact arithmetic and rigorous error bounds. We also prove the Gour--Wallach conjecture for R\'enyi entropies of all orders, with the maximiser changing from $M_4$ to cluster states at $q_*\approx1.588$, and obtain sharp Tsallis bounds, mixed-state bounds and quantitative stability.

==> four_qubit_entropy_labels.tex <==
% Generated by make_arxiv_bundle.py from four_qubit_entropy.aux: its labels, for the other document.
\newlabel{sec:fqe-intro}{{1}{1}{Introduction}{}{}}
\newlabel{fig:fqe-cuts}{{1}{3}{Four eigenvalues of each reduced density matrix for the three balanced $2|2$ cuts (same vertical scale throughout). For $M_4$ each cut has spectrum $(\tfrac 12,\tfrac 16,\tfrac 16,\tfrac 16)$ and entropy $1+\tfrac 12\log _2 3$ bits. For the cluster state $C_4$, the $12|34$ cut has spectrum $(\tfrac 12,\tfrac 12,0,0)$ and entropy $1$ bit, while the other two cuts are maximally mixed and have entropy $2$ bits, so $E(C_4)=(1+2+2)/3=5/3<E(M_4)$: balancing the three cuts beats perfecting two at the expense of one}{}{}}
\newlabel{tab:fqe-guide}{{1}{5}{Optimisers, methods and the location of complete proofs. Optimisers are listed up to local unitaries and qubit permutations; both classes attain the R\'enyi bound at $q=q_*$. Supplementary sections have an S prefix. Exact finite checks use exact arithmetic; computer-assisted proofs evaluate explicit identities in floating point with rigorous error bounds. Neither uses a numerical search as evidence. Appendix~\ref {sec:fqe-verifiers} lists the checks behind each result}{}{}}
\newlabel{tab:fqe-proof-guide}{{1}{5}{Optimisers, methods and the location of complete proofs. Optimisers are listed up to local unitaries and qubit permutations; both classes attain the R\'enyi bound at $q=q_*$. Supplementary sections have an S prefix. Exact finite checks use exact arithmetic; computer-assisted proofs evaluate explicit identities in floating point with rigorous error bounds. Neither uses a numerical search as evidence. Appendix~\ref {sec:fqe-verifiers} lists the checks behind each result}{}{}}
\newlabel{sec:fqe-main}{{2}{5}{The four-qubit maximum}{}{}}
\newlabel{thm:fqe-entropy-max}{{1}{5}{maximum and equality}{}{}}
\newlabel{tab:fqe-moment-notation}{{2}{6}{Notation for the four-qubit proof. A state is critical when all $\mathbf r_i=0$, equivalently when all one-qubit marginals are maximally mixed. Homogeneous formulas below use $N=\|z\|^2$ and unnormalised marginals; unit states have $N=1$}{}{}}
\newlabel{sec:fqe-entropy_maximum-purity-identity}{{2.1}{6}{Purity identity}{}{}}
\newlabel{lem:fqe-purity}{{2}{6}{purity identity}{}{}}
\newlabel{sec:fqe-entropy_maximum-the-sharp-moment-inequality}{{2.2}{6}{The sharp moment inequality}{}{}}
\newlabel{thm:fqe-moment}{{3}{7}{moment inequality with polarisation remainder}{}{}}
\newlabel{eq:fqe-remainder}{{{S}}{7}{The sharp moment inequality}{}{}}
\newlabel{sec:fqe-entropy_maximum-entropy-bound}{{2.3}{7}{Entropy bound}{}{}}
\newlabel{fig:fqe-majorant}{{2}{8}{The single-eigenvalue entropy contribution $f(x)=-x\ln x$ (in nats) and its cubic majorant $h$, tangent at the eigenvalues $1/6$ and $1/2$ of every cut of $M_4$. The inset magnifies the gap $h-f$ by $10^3$ on $[0.1,0.6]$: it is nonnegative, with double zeros at the nodes. Summing $h$ over the cut spectra gives an affine upper bound on the entropy in terms of $P$ and $T$; equality in this scalar bound requires every eigenvalue to be at a node}{}{}}
\newlabel{eq:fqe-entropy-gap}{{{EG}}{8}{Entropy bound}{}{}}
\newlabel{sec:fqe-entropy_maximum-equality-and-one-cut-rigidity}{{2.4}{9}{Equality and one-cut rigidity}{}{}}
\newlabel{prop:fqe-onecut}{{4}{9}{one-cut rigidity}{}{}}
\newlabel{rem:fqe-single-orbit}{{5}{9}{a single orbit}{}{}}
\newlabel{sec:fqe-spectral}{{3}{10}{R\'enyi, Tsallis and mixed-state entropies}{}{}}
\newlabel{prop:fqe-majorant}{{6}{10}{Cubic spectral majorants}{}{}}
\newlabel{eq:fqe-spectral}{{{SF}}{10}{R\'enyi, Tsallis and mixed-state entropies}{}{}}
\newlabel{cor:fqe-tsallis}{{7}{10}{Tsallis entropies}{}{}}
\newlabel{cor:fqe-renyi}{{8}{11}{R\'enyi entropies below one}{}{}}
\newlabel{cor:fqe-renyi-gw}{{9}{11}{R\'enyi envelope of Gour and Wallach}{}{}}
\newlabel{sec:fqe-spectral_corollaries-mixed-state-entanglement}{{3.1}{11}{Mixed-state entanglement}{}{}}
\newlabel{cor:fqe-convex-roof}{{10}{11}{Convex roofs}{}{}}
\newlabel{fig:fqe-renyi}{{3}{12}{Change of R\'enyi-entropy maximiser with the order $q$. The mean entropy of $M_4$ ($h_q$, solid) and that of the cluster states ($5/3$, dashed) cross once, at $q_*\approx 1.588$ (Proposition~\ref {prop:fqe-renyi-crossing}). The larger of the two, $\max \{h_q,5/3\}$, is the maximum over all pure four-qubit states (Corollary~\ref {cor:fqe-renyi-gw}): $M_4$ attains it below $q_*$ and the cluster states above $q_*$ (shaded regions). Values at $q=0$ and $q=1$ are continuous limits}{}{}}
\newlabel{sec:fqe-stability-summary}{{4}{12}{Stability of the four-qubit maximum}{}{}}
\newlabel{sec:fqe-seven-entropy}{{5}{13}{Seven qubits: compatible moments and entropy}{}{}}
\newlabel{thm:fqe-seven-purity}{{11}{13}{the seven-qubit purity minimum}{}{}}
\newlabel{thm:fqe-seven-entropy}{{12}{13}{seven-qubit mean-entropy maximum and equality}{}{}}
\newlabel{tab:fqe-seven-summary}{{3}{14}{Mean three-qubit purity and entropy of seven-qubit pure states. The AME values are not attained. The states $\Psiico $ and $\psi _{x_*}$ both lie in the icosahedral family $\psi _x$ defined below}{}{}}
\newlabel{fig:fqe-icosahedral}{{4}{14}{Icosahedral geometry and marginal spectra of $\Psiico =\psi _{37/524}$. Left: six oriented representatives of the axes through opposite icosahedral vertices label qubits $0,\ldots ,5$; the distinguished seventh qubit $s$ is separate. Dashed chords mark pairs whose amplitude sign $s_{ij}$ is $-1$. Right: spectra of the $20$ three-qubit marginals avoiding $s$ and the $15$ containing it; multiplicities in parentheses (the values $(4u)^6,(3u+x)^2$ and $8u,(4u)^5,(u+x)^2$ above at $u=15/524$); every marginal in a class has the spectrum shown. The dashed horizontal line marks the maximally mixed eigenvalue $1/8$. This state minimises the mean purity over all pure states. The entropy maximiser $\psi _{x_*}$, $x_*=0.0698\ldots $, is a different member of the same family; its spectra have the same multiplicities, and each eigenvalue differs from the one shown by less than $10^{-3}$, too little to see at this scale}{}{}}
\newlabel{eq:fqe-complex-sos}{{1}{15}{Why an icosahedron}{}{}}
\newlabel{eq:fqe-xstar}{{2}{15}{Entropy selects a different state}{}{}}
\newlabel{sec:fqe-discussion}{{6}{17}{Discussion and open problems}{}{}}
\newlabel{tab:fqe-four-seven}{{4}{18}{The copy-hierarchy method at four and seven qubits. Here $\pi _2=P/3$ and $\pi _3$ are the mean balanced cut purities. Orbits include local unitaries and qubit permutations; $\mu $ is an eigenvalue of the spin-flipped marginal}{}{}}
\newlabel{tab:fqe-other-n}{{5}{19}{Mean balanced purity and entropy of $n$-qubit pure states. With $k=\lfloor n/2\rfloor $, $\pi _k$ and $E_k$ are the mean purity and mean von Neumann entropy of the $k$-qubit marginals over all $\binom nk$ subsets of $k$ qubits. The ideal purity $2^{-k}$ and entropy $k$ are attained exactly at the AME sizes $n=2,3,5,6$. The known purity minima other than at $n=7$ are Rains linear-programming values attained by graph states (Table~\ref {tab:minima} and Theorem~\ref {thm:eighteen} of the supplement); at $n=13$ the minimum is open, and the entry is the interval of Proposition~\ref {prop:thirteeninterval} of the supplement. Single entropy entries without $<$ are exact maxima; entries with $<$ are upper bounds on unknown maxima, the ceilings $k-c_{2^k}(2^k\min \pi _k-1)$ rounded up, with the lower end of the purity interval in place of $\min \pi _k$ at $n=13$. There the maximum is open; the upper end of its interval is that ceiling, and the lower end is exceeded by an explicit state (Corollary~\ref {cor:thirteen-entropy-witness} of the supplement)}{}{}}
\newlabel{rem:fqe-spinflip-tradeoff}{{6}{19}{Purity and time reversal}{}{}}
\newlabel{sec:fqe-sextic}{{A}{20}{The sextic from elementary swap contractions}{}{}}
\newlabel{sec:fqe-sextic_identity-one-residual-tensor-and-the-local-moment-map}{{A.1}{20}{One residual tensor and the local moment map}{}{}}
\newlabel{eq:fqe-pair-norms}{{{Pr}}{20}{One residual tensor and the local moment map}{}{}}
\newlabel{eq:fqe-local-polarization}{{{U}}{21}{One residual tensor and the local moment map}{}{}}
\newlabel{sec:fqe-sextic_identity-the-three-contractions}{{A.2}{21}{The three contractions}{}{}}
\newlabel{eq:fqe-contractions}{{{C}}{21}{The three contractions}{}{}}
\newlabel{eq:fqe-antisym}{{{A}}{21}{Slot permutations}{}{}}
\newlabel{eq:fqe-kernels}{{{K}}{22}{The kernels}{}{}}
\newlabel{tab:fqe-contractions}{{6}{23}{The eleven contraction types in $\|V\|^2$. $\#$ counts the words of each type, $J$ is their mean expectation over site placements and transposition labels, and $C$ is the sum of their coefficients, so $\|V\|^2=\sum CJ$. A word acts on the three copies at each of the four sites; $I$ is the identity and $p,q,r$ are slot transpositions. Types are grouped by the number of identity letters}{}{}}
\newlabel{sec:fqe-critical-envelope}{{A.3}{24}{The critical envelope}{}{}}
\newlabel{prop:fqe-critical-envelope}{{13}{25}{critical envelope}{}{}}
\newlabel{eq:fqe-critical-envelope}{{{CE}}{25}{critical envelope}{}{}}
\newlabel{sec:fqe-sextic_identity-all-zeros-and-why-the-moment-bound-is-tight}{{A.4}{25}{All zeros and why the moment bound is tight}{}{}}
\newlabel{prop:fqe-moment-zeros}{{14}{26}{complete zero set of the moment inequality}{}{}}
\newlabel{sec:fqe-general-envelope}{{A.5}{26}{The general envelope}{}{}}
\newlabel{thm:fqe-general-envelope}{{15}{26}{general envelope and complete equality; exact certificate, FI, FG}{}{}}
\newlabel{eq:fqe-general-envelope}{{{GE}}{26}{general envelope and complete equality; exact certificate, FI, FG}{}{}}
\newlabel{sec:fqe-normal-form}{{B}{27}{Critical four-qubit states: an elementary normal form}{}{}}
\newlabel{sec:fqe-critical_four_qubit_normal_form-setting}{{B.1}{27}{Setting}{}{}}
\newlabel{eq:fqe-spin-flip-normal-form}{{{$\tau _G$}}{27}{Spin flip on the normal form}{}{}}
\newlabel{thm:fqe-critical-normal-form}{{16}{27}{Critical normal form}{}{}}
\newlabel{lem:fqe-real-gram}{{17}{27}{Simultaneous real singular values}{}{}}
\newlabel{sec:fqe-critical_four_qubit_normal_form-proof-of-theorem}{{B.2}{28}{Proof of the critical normal form}{}{}}
\newlabel{lem:fqe-moment-map}{{B.2}{28}{Proof of the critical normal form}{}{}}
\newlabel{sec:fqe-critical_four_qubit_normal_form-consequences}{{B.3}{28}{Consequences}{}{}}
\newlabel{sec:fqe-correlation}{{C}{28}{Correlation geometry of the sextic}{}{}}
\newlabel{sec:fqe-correlation_geometry-correlation-volume-identity}{{C.1}{28}{Correlation-volume identity}{}{}}
\newlabel{eq:fqe-correlation-volume}{{{CV}}{29}{Correlation-volume identity}{}{}}
\newlabel{sec:fqe-orbit-stability}{{D}{29}{Quantitative stability of the maximising LU orbits}{}{}}
\newlabel{eq:fqe-orbit-surrogate}{{3}{30}{Quantitative stability of the maximising LU orbits}{}{}}
\newlabel{thm:fqe-global-overlap}{{18}{30}{Sharp HS overlap stability}{}{}}
\newlabel{eq:fqe-global-overlap-sharp}{{4}{30}{Sharp HS overlap stability}{}{}}
\newlabel{thm:fqe-orbit-stability}{{19}{30}{Explicit global LU-orbit stability}{}{}}
\newlabel{sec:fqe-critical-orbit-stability}{{D.1}{30}{Sharp constants on the critical locus}{}{}}
\newlabel{tab:fqe-stability-scope}{{7}{31}{Distance stability: domains, constants and proof methods. The elementary polarisation and spin-flip defect bounds follow directly from \eqref {eq:fqe-entropy-gap}; they do not yet control $d$}{}{}}
\newlabel{thm:fqe-critical-orbit-sharp}{{20}{31}{Sharp critical-state orbit stability}{}{}}
\newlabel{eq:fqe-critical-fidelity}{{5}{31}{Sharp critical-state orbit stability}{}{}}
\newlabel{eq:fqe-critical-distance}{{6}{31}{Sharp critical-state orbit stability}{}{}}
\newlabel{eq:fqe-critical-entropy}{{7}{31}{Sharp critical-state orbit stability}{}{}}
\newlabel{eq:fqe-null-critical-sharp}{{8}{31}{Sharp critical-state orbit stability}{}{}}
\newlabel{eq:fqe-p1-cstar}{{9}{31}{Sharp constants on the critical locus}{}{}}
\newlabel{thm:fqe-p1-sharp}{{21}{31}{Sharp entropy stability on the critical locus}{}{}}
\newlabel{sec:fqe-orbit-consequences}{{D.2}{32}{Spectral functionals and limitations}{}{}}
\newlabel{cor:fqe-orbit-spectral}{{22}{32}{Spectral-majorant stability}{}{}}
\newlabel{sec:fqe-spectral-proofs}{{E}{32}{Proofs for R\'enyi, Tsallis and mixed-state entropies}{}{}}
\newlabel{eq:fqe-tsallis-coefficient}{{{T}}{32}{Proofs for R\'enyi, Tsallis and mixed-state entropies}{}{}}
\newlabel{eq:fqe-spectral-plus}{{{SF+}}{33}{Expanded spectral gap}{}{}}
\newlabel{sec:fqe-renyi-proofs}{{F}{34}{Proofs for R\'enyi orders above one}{}{}}
\newlabel{sec:fqe-renyi-high-order}{{F.1}{34}{High orders: an elementary bound}{}{}}
\newlabel{cor:fqe-renyi-two-up}{{23}{34}{Unrestricted high-order R\'enyi purity deficit}{}{}}
\newlabel{eq:fqe-renyi-two-up}{{{R2}}{34}{Unrestricted high-order R\'enyi purity deficit}{}{}}
\newlabel{sec:fqe-renyi-anchor-plan}{{F.2}{35}{Plan of the anchor proof}{}{}}
\newlabel{prop:fqe-renyi-crossing}{{24}{36}{HS--cluster crossing}{}{}}
\newlabel{sec:fqe-renyi-single-crossing}{{F.4}{36}{Single crossing in the order}{}{}}
\newlabel{lem:fqe-renyi-single-crossing}{{25}{36}{Single crossing}{}{}}
\newlabel{eq:fqe-renyi-single-crossing}{{{SX}}{36}{Single crossing}{}{}}
\newlabel{cor:fqe-renyi-order-transfer}{{26}{37}{Order transfer}{}{}}
\newlabel{eq:fqe-renyi-crossing-ratio}{{{SR}}{37}{Single crossing in the order}{}{}}
\newlabel{sec:fqe-quadratic-certificate}{{F.5}{38}{The universal quadratic variance bound}{}{}}
\newlabel{eq:fqe-quadratic-family}{{{QF}}{38}{The universal quadratic variance bound}{}{}}
\newlabel{thm:fqe-sharp-quadratic-variance}{{27}{38}{Sharp quadratic purity variance}{}{}}
\newlabel{eq:fqe-quadratic-variance}{{{QV}}{38}{Sharp quadratic purity variance}{}{}}
\newlabel{thm:fqe-quadratic-variance}{{28}{38}{Quadratic purity variance}{}{}}
\newlabel{eq:fqe-quadratic-variance-proved}{{{QK}}{38}{Quadratic purity variance}{}{}}
\newlabel{sec:fqe-renyi-determinant}{{F.6}{38}{Determinant reduction for four-point spectra}{}{}}
\newlabel{lem:fqe-renyi-determinant}{{29}{38}{Determinant monotonicity at fixed second and third moments}{}{}}
\newlabel{eq:fqe-renyi-double-root}{{{DM}}{38}{Determinant monotonicity at fixed second and third moments}{}{}}
\newlabel{cor:fqe-renyi-six-variable}{{30}{39}{Six-variable classical reduction}{}{}}
\newlabel{sec:fqe-renyi-cubic-bound}{{F.7}{39}{A sharp cubic R\'enyi bound from binary grouping}{}{}}
\newlabel{eq:fqe-binary-threshold}{{{BT}}{39}{A sharp cubic R\'enyi bound from binary grouping}{}{}}
\newlabel{lem:fqe-renyi-grouping}{{31}{39}{Binary grouping}{}{}}
\newlabel{eq:fqe-renyi-grouping}{{{BG}}{39}{Binary grouping}{}{}}
\newlabel{prop:fqe-cubic-bound}{{32}{40}{Sharp cubic entropy bound}{}{}}
\newlabel{eq:fqe-cubic-bound}{{{CB}}{40}{Sharp cubic entropy bound}{}{}}
\newlabel{cor:fqe-renyi-high-f}{{33}{40}{Analytic cubic envelope}{}{}}
\newlabel{eq:fqe-renyi-high-f}{{{HC}}{40}{Analytic cubic envelope}{}{}}
\newlabel{sec:fqe-renyi-covering}{{F.8}{40}{An exact Lagrangian dual for the classical relaxation}{}{}}
\newlabel{lem:fqe-dual}{{34}{40}{Lagrangian dual bound}{}{}}
\newlabel{lem:fqe-third-moment}{{35}{41}{Sharp third-moment bound at fixed purity}{}{}}
\newlabel{eq:fqe-dual-contact}{{{DC}}{41}{Exact contact identities}{}{}}
\newlabel{thm:fqe-renyi-classical}{{36}{41}{Two R\'enyi anchors}{}{}}
\newlabel{rem:fqe-renyi-covering-scope}{{37}{42}{Scope of the relaxation}{}{}}
\newlabel{sec:fqe-spectral-spinflip}{{F.9}{42}{A spectral cap from spin flip}{}{}}
\newlabel{prop:fqe-spectral-spinflip}{{38}{42}{Spectral spin-flip bound}{}{}}
\newlabel{eq:fqe-spectral-spinflip}{{10}{42}{Spectral spin-flip bound}{}{}}
\newlabel{lem:fqe-isospectral-overlap}{{39}{42}{Overlap and marginal mismatch}{}{}}
\newlabel{eq:fqe-isospectral-overlap}{{11}{42}{Overlap and marginal mismatch}{}{}}
\newlabel{eq:fqe-isospectral-rearrange}{{12}{42}{A spectral cap from spin flip}{}{}}
\newlabel{eq:fqe-isospectral-calibration}{{13}{43}{A spectral cap from spin flip}{}{}}
\newlabel{sec:fqe-renyi-two-flat}{{F.10}{43}{Quantitative rigidity of two maximally mixed cuts}{}{}}
\newlabel{prop:fqe-two-flat-rigidity}{{40}{43}{Crossed purity costs and two-flat rigidity}{}{}}
\newlabel{eq:fqe-two-flat}{{{TF}}{43}{Crossed purity costs and two-flat rigidity}{}{}}
\newlabel{sec:fqe-seven}{{G}{44}{Seven qubits: copy moments and the five-copy proofs}{}{}}
\newlabel{tab:fqe-seven-levels}{{8}{45}{The seven-qubit copy hierarchy for $\pi _3$. Strictness $L_2=1/8<L_3$ is read off the table and $L_3<L_4$ is proved (Corollary~\ref {cor:strict-copy-hierarchy} of the supplement), and $L_4<L_5$ by the exact feasible pseudo-moment of Proposition~\ref {prop:fourcopy-not-sharp} (exact certificate; checks NS-0--NS-4)}{}{}}
\newlabel{sec:ico}{{H}{46}{Seven qubits: the icosahedral state}{}{}}
\newlabel{eq:ico}{{14}{46}{Seven qubits: the icosahedral state}{}{}}
\newlabel{thm:ico}{{41}{46}{the icosahedral family}{}{}}
\newlabel{eq:icopurities}{{15}{47}{Seven qubits: the icosahedral state}{}{}}
\newlabel{cor:ico-entropy-separation}{{42}{48}{purity and entropy have different stationary points}{}{}}
\newlabel{prop:stab7}{{43}{48}{stabilizer states}{}{}}
\newlabel{sec:fqe-verifiers}{{I}{49}{Exact finite checks}{}{}}
\newlabel{tab:fqe-checks}{{9}{49}{Computer checks used by each result, by label, with their class. Section~\ref {sec:sup-verifiers} of the supplement describes each label}{}{}}

